Sphere Neural-Networks for Rational Reasoning

The success of Large Language Models (LLMs), e.g., ChatGPT, is witnessed by their planetary popularity, their capability of human-like communication, and also by their steadily improved reasoning performance. However, it remains unclear whether LLMs reason. It is an open problem how traditional neural networks can be qualitatively extended to go beyond the statistic paradigm and achieve high-level cognition. Here, we present a novel qualitative extension by generalising computational building blocks from vectors to spheres. We propose Sphere Neural Networks (SphNNs) for human-like reasoning through model construction and inspection, and develop SphNN for syllogistic reasoning, a microcosm of human rationality. SphNN is a hierarchical neuro-symbolic Kolmogorov-Arnold geometric GNN, and uses a neuro-symbolic transition map of neighbourhood spatial relations to transform the current sphere configuration towards the target. SphNN is the first neural model that can determine the validity of long-chained syllogistic reasoning in one epoch without training data, with the worst computational complexity of O(N). SphNN can evolve into various types of reasoning, such as spatio-temporal reasoning, logical reasoning with negation and disjunction, event reasoning, neuro-symbolic unification, and humour understanding (the highest level of cognition). All these suggest a new kind of Herbert A. Simon's scissors with two neural blades. SphNNs will tremendously enhance interdisciplinary collaborations to develop the two neural blades and realise deterministic neural reasoning and human-bounded rationality and elevate LLMs to reliable psychological AI. This work suggests that the non-zero radii of spheres are the missing components that prevent traditional deep-learning systems from reaching the realm of rational reasoning and cause LLMs to be trapped in the swamp of hallucination.

==> 9arxiv/abstract.tex <==
\begin{abstract} 
The success of Large Language Models (LLMs), e.g., ChatGPT, is witnessed by their planetary popularity, their capability of human-like question-answering, and also by their steadily improved reasoning performance. However, it remains unclear whether LLMs reason \cite{wei2023COT,huang2023reasoning,Mitchell_science.adj5957,chatgpt_nature2023}. It is an open problem how traditional neural networks can be qualitatively extended to go beyond the statistic paradigm and achieve high-level cognition \cite{Bengio22}. 
Here, we present a novel qualitative extension by generalising computational building blocks from vectors to spheres. Sphere boundaries introduce into contact and non-contact relations, which are primitive relations for both spatial and non-spatial reasoning \cite{Piaget69,carey09,Bellmundeaat6766,tversky19}. We propose Sphere Neural Networks (SphNNs) for human-like reasoning through model construction and inspection \cite{Jamnik01,laird2010,RagniMarkus13}, and develop  $\mathcal{S}$phNN for syllogistic reasoning, a microcosm of
human rationality \cite{Khemlani2021}. The construction is guided by a control process and a three-layered hierarchical GNN, whose middle spatial transition layer is equipped with gradual descent functions to transform spheres in the bottom layer to reach the symbolic relations in the top layer.  %Instead of training data, $\mathcal{S}$phNN uses a neuro-symbolic transition map of neighbourhood spatial relations to guide transformations from the current sphere configuration towards the target. 
$\mathcal{S}$phNN is the first neural model that can determine
the validity of long-chained syllogistic reasoning in one epoch with the worst computational complexity of ${O}(N)$ (where $N$ is the length of the chain). Experiment~\ref{exp2}demonstrates $100\%$ accuracy of $\mathcal{S}$phNN in determining the validity of every atomic syllogistic reasoning.
Compared with ChatGPT (gpt-3.5-turbo and gpt-4o) in long-chained syllogistic reasoning, $\mathcal{S}$phNN achieves $100\%$ accuracy for all $1200$ tasks, while both ChatGPT versions cannot reach $100\%$ accuracy, as shown in Experiment~\ref{exp3}. $\mathcal{S}$phNN can evaluate the answer of ChatGPT by constructing models and giving feedback through prompts, through which ChatGPT improves the accuracy in deciding the satisfiability of atomic syllogistic reasoning (Experiment~\ref{exp4}). Pre-trained vectors can be used as orientations of sphere centres, which may successfully point out target locations of spheres and tremendously shorten the time cost in sphere construction (around 90\% were shortened in Experiment ~\ref{exp5}). $\mathcal{S}$phNN can evolve into 
various types of reasoning, such as spatio-temporal reasoning, logical reasoning with negation and disjunction, event reasoning, neuro-symbolic reasoning, and humour understanding (the highest level of cognition \cite{joke2020}). All these suggest a new kind of Herbert A. Simon's scissors \cite{simon90scissor,Gigerenzer99,Gigerenzer02} with two neural blades: the representation blade using spheres to represent tasks and environments, and the reasoning blade solving problems through the transformation of sphere configurations.  
SphNNs will tremendously enhance interdisciplinary collaborations to develop the two neural blades and realise human-bounded rationality \cite{Simon19,Gigerenzer22}. This work suggests that the non-zero radii of spheres are the missing components that prevent traditional deep-learning systems from reaching the realm of rational reasoning and cause LLMs to be trapped in the swamp of hallucination. 
\end{abstract}


==> 9arxiv/experiments.tex <==
%\newpage
\section{Experiments}
   
\subsection{Experiment 1}
\label{exp2}
This experiment examines whether $\mathcal{S}$phNN can determine every {\em valid} classic syllogistic reasoning among 256 possibilities using the method of reasoning by model construction. %The out-standing result of this experiment guarantees the high quality of $\mathcal{S}$phNN for long-chained syllogistic reasoning.

\subsubsection{Method}

To determine the validity of a classic syllogistic deduction 
\syllogism{$r_1(S, M)$.\\ $r_2(M, P)$.}{$r_3(S, P)$.} $\mathcal{S}$phNN will try to refute it by constructing three spheres $\mathcal{O}_S$, $\mathcal{O}_M$, and $\mathcal{O}_P$, satisfying $\psi(r_1)(\mathcal{O}_S, \mathcal{O}_M)$, $\psi(r_2)(\mathcal{O}_M, \mathcal{O}_P)$, and $\neg\psi(r_3)(\mathcal{O}_S, \mathcal{O}_P)$. If it fails, $\mathcal{S}$phNN will conclude the original deduction is valid. The determinacy of validity requires $\mathcal{S}$phNN to construct a sphere model for each satisfiable syllogistic reasoning correctly.  

\subsubsection{Setting of experiments} We set the learning rate to 0.05, the maximum number of epochs to 1, and set different dimensions of spheres (dim) $=2, 3,15, 30, 100, 200, 2000, 10000$. All spheres are initialised as being coincided, the radius being one and the length of the centre point being 10. All experiments were conducted on MacBook Pro Apple M1 Max (10C CPU/24C GPU), 32 GB memory. 
%a personal workstation with an Intel(R) Xeon(R) E5-2640 2.40GHz CPU, and 256 GB memory. 

\subsubsection{Experiment results}  

Experiment results show that $\mathcal{S}$phNN accurately constructs Euler diagrams for each {\em satisfiable} syllogistic reasoning in the first epoch. For any syllogistic structure whose global loss is greater than zero, $\mathcal{S}$phNN concludes the premises and the negation of the conclusion is valid. This totals exactly $256-232=24$ {\em valid} syllogistic reasoning structures. This shows that the transition map of neighbourhood relations successfully guides $\mathcal{S}$phNN to construct target sphere configurations and that three control processes are effective and efficient.

\subsubsection{Discussions}
\label{discussion}


If spheres were randomly initialised, $\mathcal{S}$phNN can successfully construct Euler diagrams for all {\em satisfiable} syllogistic statements, except one as follows.
\syllogism{$all$ M are S.\\ $all$ P are M.}{$all$ S are P.}
The only model of this syllogism is all three spheres being coincided. Our strict criterion (the global loss of zero) requires $\mathcal{S}$phNN to optimise the three spheres to have the same size and to be located at the same place, which gradual descent operations are hard to construct. Consequently, $\mathcal{S}$phNN mistakenly concluded the negation of the conclusion, namely, ``some $S$ are not $P$'', is valid.  

%The exact value of $\epsilon$ is, however, related to concrete applications. %The $\epsilon$ for the molecule world shall be much smaller than the $\epsilon$ for everyday life.  



\subsection{Experiment 2}
\label{exp3}

This experiment evaluates the performance of $\mathcal{S}$phNN for long-chained syllogistic reasoning, compared with ChatGPT (``gpt-3.5-turbo''). 

\subsubsection{Testing datasets}

For syllogistic reasoning with $N$ terms, we create 24 multiple choice tasks; each task has one valid and four invalid syllogistic reasoning, totalling $24\times 5 = 120$ syllogistic reasoning tasks. We range $N$ from 3 to 12, totalling 1200 tasks. 

\subsubsection{Testing with ChatGPT and $\mathcal{S}$phNN}

We ask ChatGPT to decide the validity of syllogistic reasoning. 

For example, ``Is this reasoning always true? {\em some M1 are not S, some M2 are not M1, no M3 are M2, all P are M3, therefore, no S are P.}'' A typical answer of ChatGPT starts with its decision, followed by an explanation. 
\begin{quote}{\em
The reasoning is valid, and the conclusion is logically correct. To see why, we can draw a diagram (shown in Figure~\ref{fig:neural_diagram}(a)).
The diagram shows that there is no overlap between the S circle and the P circle and that all S are outside the P circle. This means that the statement "no S are P" is true based on the given premises.
}         
\end{quote}
We feed the same syllogistic reasoning to $\mathcal{S}$phNN, and let it decide the validity. $\mathcal{S}$phNN first negates the conclusion into {\em some S are P}, then tries to construct an Euler diagram. Finally, $\mathcal{S}$phNN successfully constructs a counter-model to refute the validity of the input syllogistic reasoning, shown in Figure~\ref{fig:neural_diagram}(b). 
\begin{figure}[h]  
\begin{subfigure}[c]{0.2\textwidth}
\includegraphics[width=0.8\textwidth]{pic/chatGPT_diagram.jpg} 
\subcaption{ChatGPT argues for the validity by showing a diagram.}
\end{subfigure}\hspace{24pt}
\begin{subfigure}[r]{0.6\textwidth}  
\centering
\includegraphics[width=1\textwidth]{pic/sphnn_diagram.jpg}
\subcaption{$\mathcal{S}$phNN refutes the validity by finding a counter Euler diagram. The circle of P, centred at $( 4.4659342765808105,1.0935691595077515 )$ with the radius $0.5761237553232794$, is part the circle of M3 that is centred at $( 4.465934753417969,1.09356689453125)$ with the radius $0.5761421616706572$.}
\end{subfigure}
\caption{Both ChatGPT and $\mathcal{S}$phNN use diagrams to check the validity of the syllogistic reasoning: {\em some M1 are not S, some M2 are not M1, no M3 are M2, all P are M3}, $\therefore$ {\em no S are P}, which is invalid.}
\label{fig:neural_diagram}
\end{figure}


\subsubsection{Testing results}
If we strictly evaluate the correctness of a {\em multiple choice} task as correctly selecting the one valid syllogism (without selecting any invalid ones), the best performance of ChatGPT is $20.1\%$ (5 among 24 tasks) when $N=3$ (classic syllogistic reasoning). If we treat one multiple choice task as five yes-no decision tasks (to decide whether syllogistic reasoning is valid), the best performance of ChatGPT is $75.0\%$ (90 among 120 tasks when $N=3$), and the performances drop to $55.0\%$ (66 among 120 tasks) as the length of chains increases, as listed in Table~\ref{chatgpt0}. 

\begin{table}[b]
\caption{Performances of {\bf ChatGPT}.}
\label{chatgpt0}
\centering
\hspace*{-1.2em}
\scalebox{0.9}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
\hline  
Syllogism with {\bf N} terms &{\bf 3}&{\bf 4} &{\bf 5}&{\bf 6}&{\bf 7}&{\bf 8}&{\bf 9}&{\bf 10}&{\bf 11}&{\bf 12}&total\\\hline 
Num. of correct multiple choices&5&5&2&3&5&3&2&1&0&1&24\\
\hline 
Num. of correct yes-no decision&90&85&75&74&83&76&71&66&66&67& 120\\
%\hline  &75.0\%&70.8\%&62.5\%&61.7\%&69.2\%&63.3\%&56.2\%&55\%&55\%&55.8\%& \\
\hline 
\end{tabular}
}
\end{table}
\begin{table}
\caption{1200 tasks are grouped by the number of terms $N$ in a reasoning task. Each group has 120 reasoning tasks. The time limit affects the performance of {\bf $\mathcal{S}$phNN}.}
\label{sphnn1}
\centering
\hspace*{-1.2em}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\hline  
time limit &{\bf N} = {\bf 3}&{\bf 4} &{\bf 5}&{\bf 6}&{\bf 7}&{\bf 8}&{\bf 9}&{\bf 10}&{\bf 11}&{\bf 12}\\\hline
$15$ (seconds) &\underline{87}&\underline{80}&60&61&48&30&27&21&12&7\\
\hline
$20$&91&88&\underline{78}&\underline{78}&64&49&46&39&25&20\\\hline
45&109&99&89&91&\underline{87}&\underline{87}&\underline{84}&\underline{76}&\underline{88}&\underline{77}\\\hline
%$75$&116&109&95&96&\underline{92}&\underline{93}&\underline{89}&\underline{85}&\underline{93}&\underline{91}\\\hline
%$135$&119&114&108&98&94&96&93&93&94&94\\\hline
$435$&{\bf 120}&{\bf 120}&118&119&118&114&109&108&101&101\\\hline
$555$&-&-&119&{\bf 120}&119&119&115&115&108&107\\\hline
$1080$&-&-&{\bf 120}&-&119&{\bf 120}&{\bf 120}&{\bf 120}&{\bf 120}&{\bf 120}\\\hline
$1200$&-&-&-&-&{\bf 120}&-&-&-&-&-\\
\hline 
\end{tabular}
}
\end{table}
In contrast, without a time limit, the performance of $\mathcal{S}$phNN is perfect. %, as listed in Table~\ref{sphnn0}. 
$\mathcal{S}$phNN does reasoning by constructing models, so generally, it needs more time for longer chained reasoning. This is also well revealed in the experiments. Table~\ref{sphnn1} listed the performance with time limits in making yes-no decisions. $\mathcal{S}$phNN can reach the performance of ChatGPT for short-chained reasoning ($N = 3, 4$) within 15 seconds, for reasoning with $N = 5, 6$ within 20 seconds. Within 45 seconds, $\mathcal{S}$phNN outperforms ChatGPT in all reasoning task groups. After around 20 minutes (1200 seconds), $\mathcal{S}$phNN can finish each reasoning task with 100\% accuracy. The random mechanism to break the coincide relations causes the construction time not proportional to the length of the reasoning task. For the task of multiple choices, $\mathcal{S}$phNN continues to outperform ChatGPT within 45 seconds. One speciality of multiple choice is that there is one and only one valid reasoning among five candidate choices. This allows $\mathcal{S}$phNN to select the right choice if it determines four among the five and reaches 100\% accuracy within a time limit of 375 seconds for each candidate choice. Table~\ref{sphnn2} listed the performance with time limits for multiple-choice tasks. 
\begin{table}[b]
\caption{The performance of $\mathcal{S}$phNN in doing multiple choice tasks.}
\label{sphnn2}
\centering
\hspace*{-1.2em}
\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\hline  
time limit &{\bf N} = {\bf 3}&{\bf 4} &{\bf 5}&{\bf 6}&{\bf 7}&{\bf 8}&{\bf 9}&{\bf 10}&{\bf 11}&{\bf 12}\\\hline
$15$ (seconds)&\underline{17}&\underline{10}&\underline{3}&3&2&0&0&0&0&0\\\hline
$20$&19&16&9&\underline{10}&\underline{7}&0&0&0&0&0\\
\hline
$45$&23&{\bf 24}&18&19&17&\underline{16}&\underline{13}&\underline{11}&\underline{17}&\underline{10}\\\hline 
$375$&{\bf 24}&-&{\bf 24}&{\bf 24}&{\bf 24}&{\bf 24}&{\bf 24}&{\bf 24}&{\bf 24}&{\bf 24}\\\hline 
\end{tabular}
}
\end{table}

\subsubsection{Analysis}

The number of possible syllogistic structures increases exponentially with the number of terms -- there are $2^{3N-1}$ different syllogistic reasoning structures for $N$ terms. It is not possible for supervised deep learning to reach the rigour of syllogistic reasoning by increasing the amount of training data. A promising alternative approach is to construct models, as advocated by main-stream cognitive psychologists, e.g., \cite{RagniMarkus13,Khemlani2021, LairdByrne91,laird87}, which ChatGPT has often used in its answers. The limitation seems to be that ChatGPT does not examine whether a model is correctly constructed. Despite this, the model-construction-styled human-like answering makes ChatGPT look professional and easily accepted. 
 
 
\subsection{Experiment 3}
\label{exp4} 

%Human-level cognition is a synergistic joint work of System 1, associative fast thinking to create coherent stories, and System 2, slow logic reasoning by following rules to check the story of System 1. Traditional deep learning is a good mirror of System 1. 
This experiment evaluates whether $\mathcal{S}$phNN can simulate the function of System 2 to provide feedback to ChatGPT, through prompt engineering to improve the performance. 


\subsubsection{The design of the experiment}

Through a well-designed prompt, we let ChatGPT decide the satisfiability of 256 types of classic syllogistic reasoning. This prompt describes the task, content, and output format in detail, so that $\mathcal{S}$phNN can easily parse the output to construct a model. The result of $\mathcal{S}$phNN will be passed to ChatGPT by appending the result to the end of the prompt. For example, to check the satisfiability of {\em 'no M0 are S', 'all P are M0', 'some S are not P'}, we feed ChatGPT the original prompt, as follows. 

\begin{verbatim}
f"""We represent '''all X are Y''' as circle X being inside
circle Y, '''no X are Y''' as circle X disconnecting from 
circle Y. '''some X are Y''' as one of the three possible 
configurations:  (1) circle X is inside circle Y; (2) circle 
X partially overlaps with circle Y; (3) circle Y is inside 
circle X. '''some X are not Y''' as one of the three possible
configurations: (1) circle X disconnects from circle Y; 
(2) circle X properly contains circle Y; (3) circle X partially
overlaps with circle Y. If '''all X are Y''', then '''some X are Y'''. 

Can the statements '''no M0 S', 'all P M0', 'some S are not P''' be 
represented by relations among three circles? 

If they cannot be represented by relations among three circles, 
only reply '''cannot''', otherwise, reply '''yes''', and give 
the relations in the list of triple forms:  
(circle X, inside, circle Y). 

Do not reply both '''cannot''' and '''yes'''.
\end{verbatim}
ChatGPT replied as follows.

\begin{verbatim}
 yes (circle s, disconnects from, circle m0), (circle p, inside,
 circle m0), (circle s, partially overlaps with, circle p)
\end{verbatim}

$\mathcal{S}$phNN checks the correctness by constructing a model\footnote{For this experiment, we extended the neuro-symbolic transition map to have the partial overlapping relation as a target relation.} for this output, and failed. This information is fed back to ChatGPT by adding the following line to the end of the above prompt. 
\begin{verbatim}
It is not correct that '''(circle s, disconnects from, 
circle m0), (circle p, inside, circle m0), (circle s, partially
overlaps with, circle p)'''
\end{verbatim}
With this feedback from $\mathcal{S}$phNN, ChatGPT repeats the task and replied, \verb+cannot+.

$\mathcal{S}$phNN then checks the satisfiability of the three original syllogistic statements {\em `no M0 are S', `all P are M0', `some S are not P'}, and concludes that they are satisfiable, so, append the following line to the end of the last prompt. 
\begin{verbatim}
It is not correct that '''cannot'''.
\end{verbatim}
With continued feedback from $\mathcal{S}$phNN, ChatGPT replied as follows.
\begin{verbatim}
Yes, the statements can be represented by relations among
three circles. The relations in the triple form are:
(circle m0, inside, circle p)
(circle s, disconnects from, circle p)
(circle s, disconnects from, circle m0)
\end{verbatim}
This time, $\mathcal{S}$phNN successfully constructed a model for the three statements from ChatGPT. After two rounds of communication with $\mathcal{S}$phNN, ChatGPT correctly answered the question. 

\subsubsection{Testing results}

We set the maximum number of communications between ChatGPT and $\mathcal{S}$phNN to 10. Without the feedback from $\mathcal{S}$phNN, ChatGPT made 207 (among 256) correct answers (80.86\%); with $\mathcal{S}$phNN's feedback, ChatGPT made 240 correct answers (93.75\%). ChatGPT's first-round answer for every 24 unsatisfiable cases was incorrect (0\%).  With the first feedback from $\mathcal{S}$phNN, ChatGPT successfully identified 22 unsatisfiable cases (91.67\%). ChatGPT failed to identify the other two unsatisfiable cases, even with ten times feedback from $\mathcal{S}$phNN. For 232 satisfiable cases, ChatGPT made 207 correct answers in the first round (89.24\%), and after ten times' feedback from $\mathcal{S}$phNN, ChatGPT made 11 more correct answers (reaching 93.97\% in accuracy), details are listed in Table~\ref{prompt}.

\begin{table}
\caption{The performance of ChatGPT supported by $\mathcal{S}$phNN.}
\label{prompt} 
\centering
\hspace*{-1.2em}
\scalebox{0.8}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline 
&
\multicolumn{1}{c}{} &\multicolumn{9}{c|}{232 satisfiable cases} &
\multicolumn{4}{c}{24 unsatisfiable cases}  \\
\hline
num. of $\mathcal{S}$phNN's feedback& 0 & 1 & 2 &3 &4 &5 & 6 &7 &9-10&0-10 & 0 & 1 & 2-10&0-10\\\hline
num. of correct answers&207 & 0& 5 &3& 1&1 &0 &1 &0 &218& 0 & 22 &0&22\\ 
\hline 
\end{tabular}
}
\end{table}

 
\subsubsection{Conclusion}

$\mathcal{S}$phNN not only successfully improves the performance of ChatGPT in deciding the satisfiability of syllogistic reasoning with three terms but also confirms the outputs of ChatGPT -- those approved by $\mathcal{S}$phNN are no more hallucinations. Our experiments show that ChatGPT is prone to answer optimistically -- for ChatGPT there are no unsatisfiable cases. Our experiments also show the first one or two rounds of feedback are especially effective and that for some tasks (16 tasks among 256), $\mathcal{S}$phNN failed to influence ChatGPT through prompt engineering. This suggests that in addition to prompt engineering, there should be other communication channels between LLMs and neural models of System 2. 


\subsection{Experiment 4}
\label{exp5}

%Compared with $\mathcal{S}$phNN in syllogistic reasoning, ChatGPT is much faster, especially for longer chains. On the other hand, $\mathcal{S}$phNN may improve the performance of ChatGPT by giving feedback through prompts, but sometimes ChatGPT ignores the message from $\mathcal{S}$phNN. 
 %-- if we fix the radii of spheres, two partially overlapped spheres will be more similar than two disconnected spheres. 
This experiment examines whether (how well) pre-trained vector embeddings can approximate orientations of the centres of spheres to construct sphere configurations. Positive experiment results will suggest three things: (1) a novel representation for neuro-symbolic unification whose centre orientations are pre-trained vectors and whose boundary relations encode symbolic relations; (2) a faster method for model construction by restricting centre orientations of spheres the same as or close to pre-trained vectors; (3) a new method of tuning pre-trained vectors by aligning them to centre orientations of a constructed model. This may lead to another effective way to communicate between LLMs and computational models of System 2.%, namely, directly optimising their interval vector embeddings by aligning them to centre orientations of spheres in a constructed model.  

\subsubsection{Testing dataset}
We group 24 {\em valid} syllogism types into 14 groups, as ``{\em no X are Y}'' has the same meaning as ``{\em no Y are X}'' and ``{\em some X are Y}'' has the same meaning as ``{\em some Y are X}''. We find 500 interpretations for each group using the hypernym relations in WordNet-3.0 \cite{MillerWordNet95},  totalling 7000 syllogism reasoning tasks. For example,   \syllogism{$\mbox{{\em all clarinetist.n.01 are musician.n.01}}$.\\$\mbox{{\em all  musician.n.01 are performer.n.01}}.$}{$\mbox{{\em  all clarinetist.n.01 are performer.n.01}}.$}
is an interpretation of the valid syllogistic reasoning 
\syllogism{$\mbox{{\em all S are M}}$.\\$\mbox{{\em all  M are P}}.$}{$\mbox{{\em  all S are P}}.$}
From the 7000 syllogistic reasoning tasks, we select those whose word stems, e.g., {\em clarinetist, musician, performer}, have different vector embeddings in 50-D GLOVE, in 1024-D BER, and in OpenAI text-embedding ada-002, totalling $2537$ tasks. Next, for each task, we enumerate the other three possible conclusions. The other three conclusions in the above example are as follows. 
\begin{enumerate}[i]
    \item \mbox{{\em some clarinetist.n.01 are not performer.n.01}}
    \item \mbox{{\em no clarinetist.n.01 are performer.n.01}}
    \item \mbox{{\em some clarinetist.n.01 are performer.n.01}}
\end{enumerate}
This totals $2537\times 4=10148$ syllogistic reasoning tasks, among which, 6479 tasks are satisfiable, and 145 tasks are interpretations of the syllogistic structure 
\syllogism{$\mbox{{\em all S are M}}$.\\$\mbox{{\em all  M are P}}.$}{$\mbox{{\em  all P are S}}.$}
or
\syllogism{$\mbox{{\em all M are P}}$.\\$\mbox{{\em all  S are M}}.$}{$\mbox{{\em  all P are S}}.$}
As observed in Experiment~\ref{exp2}, $\mathcal{S}$phNN cannot construct correct models for these 145 tasks. 
  
\subsubsection{The design of the experiment}

We create two experiment settings: (1) fix the orientation of a sphere centre to the pre-trained vector; (2) no orientation restriction and all spheres are initialised as being coincided. When the orientations of two spheres are fixed, we cannot use the constraint optimisation algorithm (Algorithm~\ref{algo:cop}), as it will cause one sphere to rotate around another sphere and change its centre orientation. We also notice that not each relation can be achieved by fixing one sphere. For example, if we fix $\mathcal{O}_V$  and the orientation of the centre of $\mathcal{O}_X$, $\mathcal{O}_X$ cannot be optimised to be inside $\mathcal{O}_V$, as illustrated in Figure~\ref{fig:exp4}. For this reason, the single relation optimisation may not be realised (in Algorithm~\ref{algo:neuro_geo}). To solve this problem, we allow iterations and set the maximum iteration number to 9. 
This way, $\mathcal{O}_X$ being inside $\mathcal{O}_V$ will be realised in the next iteration, where $\mathcal{O}_X$ is fixed, and $\mathcal{O}_V$ enlarges its radius to contain $\mathcal{O}_X$.
\begin{figure} 
\centering 
\centering
\includegraphics[width=0.5\linewidth]{pic/exp4.jpg} 
\caption{If $\mathcal{O}_V$  and the orientation of the centre of $\mathcal{O}_X$ are fixed, $\mathcal{O}_X$ cannot be inside $\mathcal{O}_V$.}
\label{fig:exp4}
\end{figure}

\begin{table}
\caption{The orientation of pre-trained vectors very well approximates the orientation of spheres}
\label{ptv} 
\centering
\hspace*{-1.2em}
\scalebox{0.8}{
\begin{tabular}{c|c|c|c}
\hline 
\multicolumn{3}{c|}{using pre-trained vectors as the orientations of centres} &
\multicolumn{1}{c}{no restrictions}  \\
\hline
GLOVE 50-D &BERT 1024-D& OpenAI text-embedding ada-002 & all spheres are initialised as being coincided\\\hline
6479/6624 & 6479/6624 &6479/6624 &6624/6624\\ 
\hline 
$97.81\%$ & $97.81\%$ & $97.81\%$ & $100.00\%$ \\ 
\hline 
\end{tabular}
}
\end{table}


\subsubsection{Experiment results and analysis}

Without restriction, $\mathcal{S}$phNN successfully constructed models for every satisfiable syllogistic reasoning (6624 tasks). When orientations of sphere centres are fixed to pre-trained vectors, $\mathcal{S}$phNN successfully constructed models for all 6479 tasks, with 145 unsuccessful cases, as expected. Results are listed in shown in Table~\ref{ptv}. 

 

==> 9arxiv/quote.tex <==
\begin{quote}
\centering
    {\em The origin of reason is gradually developed. 
    
    \hfill --- Charles Darwin 
        } 
\end{quote}

\begin{quote} 
{\em 
Spatial thinking is the foundation of abstract thought.
    
    \hfill --- Barbara Tversky  \cite{tversky19}
     } 
\end{quote}

\begin{quote} 
{\em 
We conceive GPS as moving through
a large maze. The nodes of the maze represent situations, described afferently; the paths joining one node to another are the actions, described as
motor sequences, that will transform the one situation into the other. At
any given moment GPS is always faced with a single question: ``What
action shall I try next?''
    
    \hfill --- Herbert A. Simon  \cite{Simon19}
     } 
\end{quote}

 
\begin{quote}
    {\em  What we will put to you, then, is an interactionist approach to reason that contrasts with standard intellectualist approaches. 
   \begin{flushright} --- Mercier and Sperber \cite{enigma2018}
        \end{flushright}
    }
\end{quote}

\begin{quote} 
{\em 
It seems impossible to reach any definitive conclusions concerning human rationality in the absence of a detailed analysis of the sensitivity of the criterion and the cost involved in evaluating the alternatives.  
    
    \hfill --- Amos Tversky  \cite{Tversky69}
     } 
\end{quote}

 \begin{quote}
    {\em 
Automatic inference in perception and deliberate inference in reasoning are at the two ends of a continuum. Between them, there is a great variety of inferential processes doing all kinds of jobs. 

\hfill--- Mercier and Sperber  \cite{enigma2018}

        }
\end{quote}


\begin{quote} 
    {\em The intuitive mind is a sacred gift and the rational mind is a faithful servant. 
    
    \hfill ---Albert Einstein  
        } 
\end{quote}
